A Galaxy-Targeted Search for the Optical Counterpart of the Candidate NS-BH Merger S190814bv with Magellan

On 2019 August 14 the Laser Interferometer Gravitational Wave Observatory (LIGO) and the Virgo gravitational wave interferometer announced the detection of a binary merger, S190814bv, with a low false alarm rate (FAR) of about 1 in $1.6\times 10^{25}$ years, a distance of $267\pm 52$ Mpc, a 90\% (50\%) localization region of about 23 (5) deg$^2$, and a probability of being a neutron star--black hole (NS-BH) merger of $>99\%$. The LIGO/Virgo Collaboration (LVC) defines NS-BH such that the lighter binary member has a mass of $<3$ M$_\odot$ and the more massive one has $>5$ M$_\odot$, and this classification is in principle consistent with a BH-BH merger depending on the actual upper mass cut-off for neutron stars. Additionally, the LVC designated a probability that the merger led to matter outside the final BH remnant of $<1\%$, suggesting that an electromagnetic (EM) counterpart is unlikely. Here we report our optical follow-up observations of S190814bv using the Magellan Baade 6.5 m telescope to target all 96 galaxies in the GLADE catalog within the 50\% localization volume (representing about 70\% of the integrated luminosity within this region). No counterpart was identified to a median $3\sigma$ limiting magnitude of $i=22.2$ ($M_i\approx -14.9$ mag), comparable to the brightness of the optical counterpart of the binary neutron star merger GW170817 at the distance of S190814bv; similarly, we can rule out an on-axis jet typical of short GRBs. However, we cannot rule out other realistic models, such as a kilonova with only $\sim 0.01$ M$_\odot$ of lanthanide-rich material, or an off-axis jet with a viewing angle of $\theta_{\rm obs}\gtrsim 15^\circ$.

==> mycommands.tex <==
% New Commands
\newcommand{\tc}[2][red]{\textcolor{#1}{\emph{\textbf{#2}}}}
\newcommand{\ksmag}{\emph{Ks}~magnitudes }
\newcommand{\jmag}{\emph{J}~magnitudes }
\newcommand{\kpmags}{\emph{Kp}~magnitudes }
\newcommand{\kpmag}{\emph{Kp}~magnitude }
\newcommand{\teff}{\ensuremath{T_{\mathrm{eff}}}}
\newcommand{\logg}{\ensuremath{\log g}}
\newcommand{\kepler}{{\em Kepler}\xspace}
\def\msun{{\rm\,M_\odot}}
\def\rsun{{\rm\,R_\odot}}
\def\mearth{{\rm\,M_\oplus}}
\def\rearth{{\rm\,R_\oplus}}
\def\fearth{{\rm\,F_\oplus}}
\def\lsun{{\rm\,L_\odot}}
\newcommand{\hho}{H$_2$O}
\newcommand{\hh}{H$_2$}
\newcommand{\oo}{O$_2$}
\newcommand{\chhhh}{CH$_4$}
\newcommand{\mjup}{{\rm M}_{\rm Jup}}
\newcommand{\kms}{\rm km\ s^{-1}}
\newcommand{\mps}{\rm m\ s^{-1}}
\newcommand{\cspg}{\rm\ cm^2\ g^{-1}}
\newcommand{\ergs}{\rm\ erg\ s^{-1}}
\newcommand{\kelvin}{\rm K}
\newcommand{\angstrom}{\rm \AA}
\newcommand{\oneday}{\rm day}
\newcommand{\days}{\rm days}
\newcommand{\hours}{\rm hours}
\newcommand{\meter}{\rm m}
\newcommand{\HST}{{\it HST}}
\newcommand{\hubble}{{\it HST}}
\newcommand{\spitzer}{{\it Spitzer}}
\newcommand{\fermi}{{\it Fermi}}
\newcommand{\swift}{{\it Swift}}
\newcommand{\gaia}{{\it Gaia}}
\newcommand{\mosfit}{{\tt MOSFiT}}
\newcommand{\zeroth}{$0^{\rm th}$}
\newcommand{\first}{$1^{st}$}
\newcommand{\second}{$2^{nd}$}
\newcommand{\third}{$3^{rd}$}
\newcommand{\fourth}{$4^{th}$}
\newcommand{\e}{${\rm e^{-}}$}
\newcommand{\persecond}{${\rm s^{-1}}$}
\newcommand{\perpixel}{${\rm pixel^{-1}}$}
\newcommand{\divideoot}{{\tt divide-oot}}
\newcommand{\modelramp}{{\tt model-ramp}}
\newcommand{\chisq}{$\chi^2$}
\newcommand{\calwf}{{\tt calwf3}}
\newcommand{\rp}{$R_{p}$}
\newcommand{\rs}{$R_{\star}$}
\newcommand{\flt}{{\tt flt}}
\definecolor{orange}{rgb}{.8,0.4,0}
\newcommand{\question}[1]{\sffamily {\em {\color{orange} [#1]}}\normalfont}
\newcommand{\todo}[1]{\sffamily {\em {\color{orange} #1}}\normalfont}
\newcommand{\mad}{\rm MAD}
\newcommand{\Mej}{M_{\rm ej}}
\newcommand{\vej}{v_{\rm ej}}
\newcommand{\apx}{\ensuremath{\sim}}
\newcommand{\WFDD}{{\tt WFDD}}
\newcommand{\WFDM}{{\tt WFDM}}
\newcommand{\WFDR}{{\tt WFDR}}

% Alternate Itemize
\newcommand{\outline}[1]{
\todo{\begin{itemize}
#1
\end{itemize}}}

% AutoRef Stuff
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\subsubsectionautorefname{Section}

\renewcommand*{\sectionautorefname}{Section} 
\renewcommand*{\subsectionautorefname}{Section} 

% Citation Alias
\defcitealias{LP98}{LP98}
\defcitealias{CowpBerger15}{CB15}

